Early Detection of Research Trends

Being able to rapidly recognise new research trends is strategic for many stakeholders, including universities, institutional funding bodies, academic publishers and companies. The literature presents several approaches to identifying the emergence of new research topics, which rely on the assumption that the topic is already exhibiting a certain degree of popularity and consistently referred to by a community of researchers. However, detecting the emergence of a new research area at an embryonic stage, i.e., before the topic has been consistently labelled by a community of researchers and associated with a number of publications, is still an open challenge. In this dissertation, we begin to address this challenge by performing a study of the dynamics preceding the creation of new topics. This study indicates that the emergence of a new topic is anticipated by a significant increase in the pace of collaboration between relevant research areas, which can be seen as the 'ancestors' of the new topic. Based on this understanding, we developed Augur, a novel approach to effectively detecting the emergence of new research topics. Augur analyses the diachronic relationships between research areas and is able to detect clusters of topics that exhibit dynamics correlated with the emergence of new research topics. Here we also present the Advanced Clique Percolation Method (ACPM), a new community detection algorithm developed specifically for supporting this task. Augur was evaluated on a gold standard of 1,408 debutant topics in the 2000-2011 timeframe and outperformed four alternative approaches in terms of both precision and recall.

==> front-matter/acronyms.tex <==
    \chapter*{Acronyms}
    \begin{acronym}[UMLX]
        \acro{DRY}{Don't Repeat Yourself}
        \acro{API}{Application Programming Interface}
        \acro{UML}{Unified Modeling Language}
    \end{acronym} 

==> front-matter/thesis-info.tex <==
% ************************ Thesis Information & Meta-data **********************
%% The title of the thesis
\title{Explaining Data Patterns using Knowledge from the Web of Data}
%\texorpdfstring is used for PDF metadata. Usage:
%\texorpdfstring{LaTeX_Version}{PDF Version (non-latex)} eg.,
%\texorpdfstring{$sigma$}{sigma}

%% Subtitle (Optional)
%\subtitle{How Linked Data background knowledge to automatically explain Knowledge Discovery patterns}

%% The full name of the author
\author{Angelo Salatino}

%% Department (eg. Department of Engineering, Maths, Physics)
\dept{Knowledge Media Institute}

%% University and Crest
\university{The Open University}
% Crest minimum should be 30mm.
\crest{\includegraphics[width=0.2\textwidth]{OU-logo}}

%% Use this crest, if you are using the college crest
%% Crest long miminum should be 65mm
%\crest{\includegraphics[width=0.45\textwidth]{University_Crest_Long}}

%% College shield [optional] 
% Crest minimum should be 30mm.
\collegeshield{\includegraphics[width=0.25\textwidth]{kmi-logo}}

%% You can redefine the submission text:
% Default as per the University guidelines:
% ``This dissertation is submitted for the degree of''
%\renewcommand{\submissiontext}{change the default text here if needed}

%% Full title of the Degree
\degreetitle{Doctor of Philosophy}



%% Submission date
% Default is set as {\monthname[\the\month]\space\the\year}
%\degreedate{September 2014} 

%% Meta information
%\subject{LaTeX} \keywords{{LaTeX} {PhD Thesis} {Engineering} {University of
%Cambridge}}

